Cross-Correlated Attention Networks for Person Re-Identification

Deep neural networks need to make robust inference in the presence of occlusion, background clutter, pose and viewpoint variations -- to name a few -- when the task of person re-identification is considered. Attention mechanisms have recently proven to be successful in handling the aforementioned challenges to some degree. However previous designs fail to capture inherent inter-dependencies between the attended features; leading to restricted interactions between the attention blocks. In this paper, we propose a new attention module called Cross-Correlated Attention (CCA); which aims to overcome such limitations by maximizing the information gain between different attended regions. Moreover, we also propose a novel deep network that makes use of different attention mechanisms to learn robust and discriminative representations of person images. The resulting model is called the Cross-Correlated Attention Network (CCAN). Extensive experiments demonstrate that the CCAN comfortably outperforms current state-of-the-art algorithms by a tangible margin.

==> paper_graphical_abstract.tex <==
% \section*{Graphical Abstract (Optional)}
% To create your abstract, please type over the instructions in the
% template box below.  Fonts or abstract dimensions should not be changed
% or altered. 

% \vskip1pc
% \fbox{
% \begin{tabular}{p{.4\textwidth}p{.5\textwidth}}
% \bf Type the title of your article here  \\
% Author's names here \\[1pc]
% \includegraphics[width=.3\textwidth]{top-elslogo-fm1}%%.pdf
% & 
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% This is the dummy text for graphical abstract.
% %}\\
% \end{tabular}
% }

% \end{table*}

% \clearpage
% \thispagestyle{empty}

% \ifpreprint
%   \vspace*{-1pc}
% \else
% %  \vspace*{-6pc}
% \fi

% \begin{table*}[!t]
% \ifpreprint\else\vspace*{-15pc}\fi

\section*{Research Highlights (Required)}

To create your highlights, please type the highlights against each
\verb+\item+ command. 

\vskip1pc

\fboxsep=6pt
\fbox{
\begin{minipage}{.95\textwidth}
It should be short collection of bullet points that convey the core
findings of the article. It should  include 3 to 5 bullet points
(maximum 85 characters, including spaces, per bullet point.)  
\vskip1pc
\begin{itemize}

 \item 

 \item 

 \item

 \item

 \item

\end{itemize}
\vskip1pc
\end{minipage}
}

% \end{table*}

% \clearpage


\ifpreprint
  \setcounter{page}{1}
\else
  \setcounter{page}{1}
\fi

